Robust Fine-tuning of Zero-shot Models via Variance Reduction

When fine-tuning zero-shot models like CLIP, our desideratum is for the fine-tuned model to excel in both in-distribution (ID) and out-of-distribution (OOD). Recently, ensemble-based models (ESM) have been shown to offer significant robustness improvement, while preserving high ID accuracy. However, our study finds that ESMs do not solve the ID-OOD trade-offs: they achieve peak performance for ID and OOD accuracy at different mixing coefficients. When optimized for OOD accuracy, the ensemble model exhibits a noticeable decline in ID accuracy, and vice versa. In contrast, we propose a sample-wise ensembling technique that can simultaneously attain the best ID and OOD accuracy without the trade-offs. Specifically, we construct a Zero-Shot Failure (ZSF) set containing training samples incorrectly predicted by the zero-shot model. For each test sample, we calculate its distance to the ZSF set and assign a higher weight to the fine-tuned model in the ensemble if the distance is small. We term our method Variance Reduction Fine-tuning (VRF), as it effectively reduces the variance in ensemble predictions, thereby decreasing residual error. On ImageNet and five derived distribution shifts, our VRF further improves the OOD accuracy by 1.5 - 2.0 pp over the ensemble baselines while maintaining or increasing ID accuracy. VRF achieves similar large robustness gains (0.9 - 3.1 pp) on other distribution shifts benchmarks. Codes are available in https://github.com/BeierZhu/VRF.

==> images/Distance-to-ZSF-others.tex <==
\begin{figure}[t]
    \centering
\includegraphics[width=1.\textwidth]{images/distance-to-ZSF-others.pdf}
    \caption{ Relationship between the ratio of fine-tuning accuracy to zero-shot accuracy $\frac{\text{Acc}_\mathsf{ft}}{\text{Acc}_\mathsf{zs}}$ and the distance to the zero-shot failure set ($d(\x)$). (a) CIFAR-10 and STL-10 results. (b) Entity-30 results.
    }
\label{fig:dist-to-ZSF-others}
\end{figure}


==> images/ID-OOD-frontiers-others.tex <==
\begin{figure}[t]
    \centering
\includegraphics[width=1.\textwidth]{images/id-ood-frontier-others.pdf}
    \caption{ ID-OOD frontier curves for the CLIP ViT-B/16 by varing the mixing coefficient $\alpha$. (a) CIFAR-10 (ID) and STL-10 (OOD) results. (b) Entity-30 results.
    }
\label{fig:id-ood-others}
\end{figure}


==> sections/7-acknowledge.tex <==
\section*{Acknowledgments}
This research is supported by the National Research Foundation, Singapore
under its AI Singapore Programme (AISG Award No: AISG2-PhD-2021-01-002 and AI Singapore AISG2-RP-2021-022). 

==> sections/depricated.tex <==
\subsection{Variance Reduction Fine-tuning Leads to Lower Residual Error}
Let us shift our focus to the effects of combining the zero-shot and fine-tuned models. 
Let $g_\mathsf{zs}(\cdot)$ and $g_\mathsf{ft}(\cdot)$ be two functions that produce weights for ensembling the models. Under the constraint that $g_\mathsf{zs}(\x) + g_\mathsf{ft}(\x)=1$,
the residual error of the combined classifier is obtained by:
\begin{equation}
    \hat{\mathbb{P}}_\mathsf{vrf}(y|\x)=g_\mathsf{zs}(\x) \hat{\mathbb{P}}_\mathsf{zs}(y|\x) + g_\mathsf{ft}(\x) \hat{\mathbb{P}}_\mathsf{ft}(y|\x)  =\mathbb{P}(y|\x) + \underbrace{g_\mathsf{zs}(\x)\cdot \eta_\mathsf{zs}(\x) + g_\mathsf{ft}(\x)\cdot \eta_\mathsf{ft}(\x)}_{\eta_\mathsf{vrf}(\x)} ,
\end{equation}
where we omit the subscript $y$ of $\eta$ for readability. The variance of $\eta_\mathsf{vrf}(\x)$ can be expressed as:
\begin{equation}\label{eq:fullvar}
    \mathbb{V}[\eta_\mathsf{vrf}(\x)]=g_\mathsf{zs}(\x)^2\cdot \mathbb{V}[\eta_\mathsf{zs}(\x)] + g_\mathsf{ft}(\x)^2\cdot \mathbb{V}[\eta_\mathsf{ft}(\x)] + 2 \cdot g_\mathsf{zs}(\x)\cdot g_\mathsf{ft}(\x)\cdot \mathbb{C}[\eta_\mathsf{zs}(\x),\eta_\mathsf{ft}(\x)].
\end{equation}
$\mathbb{C}[\eta_\mathsf{zs}(\x),\eta_\mathsf{ft}(\x)]$ is the covariance between $\eta_\mathsf{zs}(\x)$ and $\eta_\mathsf{ft}(\x)$. Previous studies~\cite{wortsman2022robust,zhu2024generalized} observe an empirical phenomena that the zero-shot and the fine-tuned models have diverse predictions. We further re-exam this finding in Section~\ref{sec:abla} and find a very low correlation between $\eta_\mathsf{zs}(\x)$ and $\eta_\mathsf{ft}(\x)$ (Pearson coefficient $\rho \approx 0.05$). Therefore, we focus on the first two terms in Eq.~\eqref{eq:fullvar} and omit the covariance term:
\begin{equation}\label{eq:simplevar}
    \mathbb{V}[\eta_\mathsf{vrf}(\x)] \approx g_\mathsf{zs}(\x)^2\cdot \mathbb{V}[\eta_\mathsf{zs}(\x)] + g_\mathsf{ft}(\x)^2\cdot \mathbb{V}[\eta_\mathsf{ft}(\x)].
\end{equation}
According to Eq.~\eqref{eq:var-error}, the reduction in variance can be readily translated into a reduction in error rates. To obtain the smallest variance $\mathbb{V}[\eta_\mathsf{vrf}(\x)]$, we minimize Eq.~\eqref{eq:simplevar} using Lagrange multiplier to enforce the constraint that $g_\mathsf{zs}(\x) + g_\mathsf{ft}(\x)=1$, and obtain the optimal weight function $g_\mathsf{ft}$ as:
\begin{equation}
     g_\mathsf{ft}(\x)=\frac{\mathbb{V}[\eta_\mathsf{zs}(\x)]}{\mathbb{V}[\eta_\mathsf{zs}(\x)] + \mathbb{V}[\eta_\mathsf{ft}(\x)]}=\frac{E_\mathsf{zs}}{E_\mathsf{zs}+E_\mathsf{ft}}=(1+\frac{E_\mathsf{ft}}{E_\mathsf{zs}})^{-1} \propto \frac{\text{Acc}_\mathsf{ft}}{\text{Acc}_\mathsf{zs}}
\end{equation}
Since $\frac{\text{Acc}_\mathsf{ft}}{\text{Acc}_\mathsf{zs}} \propto d(\x)^{-1}$ (a smaller distance $d(\x)$ associated with a larger $\frac{\text{Acc}_\mathsf{ft}}{\text{Acc}_\mathsf{zs}}$ as shown in Fig.~\ref{fig:ft_zc_w}), we design the weighting function $g_\mathsf{ft}(\x)=\omega(\x)  \propto d(\x)^{-1} $ as in Eq.~\eqref{eq:weight}.  
